DeepCut: Joint Subset Partition and Labeling for Multi Person Pose Estimation

This paper considers the task of articulated human pose estimation of multiple people in real world images. We propose an approach that jointly solves the tasks of detection and pose estimation: it infers the number of persons in a scene, identifies occluded body parts, and disambiguates body parts between people in close proximity of each other. This joint formulation is in contrast to previous strategies, that address the problem by first detecting people and subsequently estimating their body pose. We propose a partitioning and labeling formulation of a set of body-part hypotheses generated with CNN-based part detectors. Our formulation, an instance of an integer linear program, implicitly performs non-maximum suppression on the set of part candidates and groups them to form configurations of body parts respecting geometric and appearance constraints. Experiments on four different datasets demonstrate state-of-the-art results for both single person and multi person pose estimation. Models and code available at http://pose.mpi-inf.mpg.de.

==> ap-det-roi-0.5-0.2-expidx477.tex <==
Fast R-CNN \detroi~\textcolor{red}{391} & 57.7  & 49.7  & 32.8  & 21.3  & 25.0  & 20.4 & 13.0 & 40.4 & 32.0 \\



==> ap-det-roi-0.5-0.2-expidx479.tex <==
Fast R-CNN \detroi~\textcolor{red}{1737}& 58.6  & 49.2  & 32.4  & 19.0  & -  & - & - & 39.8 & - \\



==> ap-det-roi-0.5-0.2-expidx485.tex <==
Fast R-CNN \detroi~\textcolor{red}{76} & 62.0  & 55.4  & 42.6  & 29.5  & 33.4  & 25.3 & 16.9 & 47.4 & 38.5 \\



==> ap-det-roi-0.5-0.2-expidx486.tex <==
Fast R-CNN \detroi~\textcolor{red}{840}& 64.5  & 58.5  & 39.7  & 27.4  & - & - & - & 47.5 & - \\



==> ap-det-roi-0.5-0.2-nimg103-expidx485.tex <==
Fast R-CNN \detroi& 72.0  & 68.4  & 55.2  & 35.8  & 47.1  & 35.5 & 22.0 & 57.8 & 48.6 \\



==> ap-det-roi-0.5-0.2-nimg103-expidx486.tex <==
Fast R-CNN \multbu& 72.4  & 68.8  & 54.6  & 35.3  & -  & - & - & 57.8 & - \\



==> ap-det-roi-0.5-0.2-nimg103-expidx498.tex <==
Dense \detroi& 78.2  & 75.9  & 61.6  & 43.7  & 53.1  & 41.5 & 33.0 & 64.8 & 55.9 \\



==> ap-det-roi-0.5-0.2-nimg103-expidx500.tex <==
Dense \multbu& 78.2  & 75.8  & 62.1  & 47.4  & -  & - & - & 65.9 & - \\



==> ap-det-roi-0.5-0.2-nimg162-expidx485.tex <==
\rcnn~\detroi& 70.2  & 64.7  & 50.8  & 34.7  & 45.9  & 36.6 & 20.8 & 55.1 & 46.8 \\



==> ap-det-roi-0.5-0.2-nimg162-expidx486.tex <==
Fast R-CNN \multbu& 71.9  & 66.3  & 50.5  & 34.7  & -  & - & - & 55.8 & - \\



==> ap-det-roi-0.5-0.2-nimg162-expidx498.tex <==
\dense~\detroi& 75.3  & 71.1  & 57.9  & 42.9  & 53.5  & 37.8 & 28.3 & 61.8 & 53.0 \\



==> ap-det-roi-0.5-0.2-nimg162-expidx500.tex <==
Dense \detroi& 76.9  & 73.4  & 59.2  & 45.8  & -  & - & - & 63.8 & - \\



==> ap-det-roi-0.5-0.2-nimg288-expidx486.tex <==
Fast R-CNN \multbu& 73.5  & 67.8  & 49.9  & 33.9  & -  & - & - & 56.3 & - \\



==> ap-det-roi-0.5-0.2-nimg288-expidx500.tex <==
Dense \multbu& 79.1  & 74.4  & 57.6  & 44.6  & -  & - & - & 63.9 & - \\



==> ap-det-roi-expidx477.tex <==
Fast R-CNN \detroi& 48.1  & 42.6  & 30.9  & 19.2  & 23.1  & 15.9 & 11.1 & 35.2 & 27.8 \\



==> ap-expidx477.tex <==
Fast R-CNN \multb~\textcolor{red}{391} & 51.2  & 47.3  & 34.9  & 23.1  & 27.9  & 21.7 & 14.5 & 39.1 & 32.0 \\



==> ap-expidx479.tex <==
Fast R-CNN \multbu~\textcolor{red}{1737}& 58.2  & 49.8  & 33.3  & 21.7  & -  & - & - & 40.8 & -\\



==> ap-expidx485.tex <==
Fast R-CNN \multb~\textcolor{red}{76}& 63.5  & 56.5  & 44.2  & 30.1  & 37.4  & 26.6 & 25.5 & 48.6 & 41.1 \\



==> ap-expidx486.tex <==
Fast R-CNN \multbu~\textcolor{red}{840}& 66.4  & 60.1  & 44.9  & 30.5  & -  & - & - & 50.5 & - \\



==> ap-expidx487.tex <==
mpii multi& 40.3  & 23.5  & 13.2  & 8.7  & 12.4  & 8.5 & 5.4 & 21.4 & 16.4 & NaN \\



==> ap-expidx695-GT.tex <==
Dense \gtroi~\textcolor{red}{408}& 74.5  & 69.7  & 59.3  & 48.5  & 51.8  & 47.5 & 44.9 & 63.0 & 57.0 \\


==> ap-expidx695-det.tex <==
Dense \detroi~\textcolor{red}{408} & 67.5  & 64.8  & 50.5  & 36.6  & 48.3  & 37.8 & 26.7 & 54.8 & 47.9 \\


==> ap-expidx695.tex <==
Dense \multb~\textcolor{red}{408} & 68.1  & 64.4  & 50.7  & 35.2  & 49.5  & 39.0 & 28.8 & 54.6 & 48.4  \\


==> ap-expidx699.tex <==
Dense \multbu~\textcolor{red}{522} & 76.2  & 68.8  & 58.6  & 44.7  & -  & - & - & 62.1 & - \\
Dense \gtroi~\multbu~\textcolor{red}{522} & 78.4  & 71.4  & 60.3  & 51.7  & -  & - & - & 65.4 & - \\


==> ap-gt-roi-expidx477.tex <==
Fast R-CNN \gtroi~\textcolor{red}{391} & 61.1  & 52.2  & 38.9  & 29.8  & 30.5  & 26.3 & 22.9 & 45.5 & 37.9 \\



==> ap-gt-roi-expidx479.tex <==
Fast R-CNN \gtroi~\textcolor{red}{1737}& 63.8  & 54.7  & 39.0  & 30.0  & -  & - & - & 46.9 & - \\



==> ap-gt-roi-expidx485.tex <==
Fast R-CNN \gtroi~\textcolor{red}{76}& 64.6  & 58.1  & 46.1  & 35.9  & 36.6  & 28.6 & 21.4 & 51.2 & 42.2 \\



==> ap-gt-roi-expidx486.tex <==
Fast R-CNN \gtroi~\textcolor{red}{840}& 68.1  & 60.6  & 45.8  & 37.0  & -  & - & - & 52.9 & - \\



==> ap-gt-roi-nimg103-expidx485.tex <==
Fast R-CNN \gtroi& 72.9  & 67.5  & 57.1  & 43.4  & 50.1  & 44.3 & 38.2 & 60.2 & 53.8 \\



==> ap-gt-roi-nimg103-expidx486.tex <==
Fast R-CNN \multbu& 73.1  & 66.2  & 59.0  & 43.6  & -  & - & - & 60.5 & - \\



==> ap-gt-roi-nimg103-expidx498.tex <==
Dense \gtroi& 75.8  & 77.2  & 64.6  & 52.6  & 55.9  & 47.7 & 45.0 & 67.6 & 60.4 \\



==> ap-gt-roi-nimg103-expidx500.tex <==
Dense \multbu& 76.5  & 76.9  & 64.8  & 54.1  & -  & - & - & 68.1 & - \\



==> ap-gt-roi-nimg162-expidx485.tex <==
\rcnn~\gtroi& 72.0  & 64.1  & 54.8  & 44.1  & 48.5  & 45.4 & 38.4 & 58.8 & 52.9 \\



==> ap-gt-roi-nimg162-expidx486.tex <==
Fast R-CNN \multbu& 73.9  & 63.8  & 56.3  & 44.3  & -  & - & - & 59.6 & - \\



==> ap-gt-roi-nimg162-expidx498.tex <==
\dense~\gtroi& 76.2  & 74.0  & 64.6  & 53.4  & 56.3  & 46.2 & 44.7 & 67.0 & 59.8 \\



==> ap-gt-roi-nimg162-expidx500.tex <==
Dense \gtroi& 77.6  & 75.3  & 65.4  & 56.0  & -  & - & - & 68.6 & - \\



==> ap-gt-roi-nimg288-expidx486.tex <==
Fast R-CNN \multbu& 75.0  & 67.4  & 55.7  & 43.3  & -  & - & - & 60.4 & - \\



==> ap-gt-roi-nimg288-expidx500.tex <==
Dense \multbu& 79.4  & 75.6  & 64.3  & 55.6  & -  & - & - & 68.7 & - \\



==> ap-nimg103-expidx485.tex <==
Fast R-CNN \multb& 73.5  & 68.6  & 58.0  & 39.7  & 49.6  & 39.8 & 26.9 & 60.0 & 51.5 \\



==> ap-nimg103-expidx486.tex <==
Fast R-CNN \multbu& 74.6  & 71.4  & 61.3  & 39.5  & -  & - & - & 61.7 & - \\



==> ap-nimg103-expidx498.tex <==
Dense \multb& 76.2  & 76.1  & 62.0  & 38.4  & 57.3  & 48.0 & 33.3 & 63.2 & 56.4 \\



==> ap-nimg103-expidx500.tex <==
Dense \multbu& 82.8  & 80.4  & 67.6  & 55.8  & -  & - & - & 71.7 & - \\



==> ap-nimg162-expidx485.tex <==
\deepcut~\multb~\rcnn& 72.1  & 65.6  & 54.9  & 39.4  & 48.8  & 40.4 & 29.4 & 58.0 & 50.6 \\



==> ap-nimg162-expidx486.tex <==
\deepcut~\multbu~\rcnn& 73.9  & 69.1  & 56.9  & 39.6  & -  & - & - & 59.9 & - \\



==> ap-nimg162-expidx498.tex <==
\deepcut~\multb~\dense& 72.2  & 71.6  & 60.4  & 41.5  & 54.9  & 45.4 & 32.6 & 61.4 & 54.6 \\



==> ap-nimg162-expidx500.tex <==
\deepcut~\multbu~\dense& 79.7  & 75.8  & 64.8  & 52.6  & -  & - & - & 68.2 & - \\



==> figure_qualitative_mpii_supplemental_all.tex <==
\begin{figure*}
  \centering
  \begin{tabular}{c c c c c c}

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0013_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0013_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0013_sticks.pdf}&

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0231_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0231_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0231_sticks.pdf}\\

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0405_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0405_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0405_sticks.pdf}&

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0564_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0564_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0564_sticks.pdf}\\

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0630_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0630_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0630_sticks.pdf}&

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0953_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0953_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0953_sticks.pdf}\\

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0960_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0960_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0960_sticks.pdf}&

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1025_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1025_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1025_sticks.pdf}\\

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1620_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1620_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1620_sticks.pdf}&

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1621_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1621_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1621_sticks.pdf}\\

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0488_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0488_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0488_sticks.pdf}&

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0311_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0311_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0311_sticks.pdf}\\

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1680_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1680_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1680_sticks.pdf}&

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1692_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1692_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1692_sticks.pdf}\\

  \end{tabular}
  \label{fig:qualitative_mpii}
\end{figure*}

\begin{figure*}
  \centering
  \begin{tabular}{c c c c c c}


\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0695_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0695_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0695_sticks.pdf}&

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1346_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1346_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1346_sticks.pdf}\\

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1253_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1253_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1253_sticks.pdf}&

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1674_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1674_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1674_sticks.pdf}\\

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0908_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0908_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0908_sticks.pdf}&

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0104_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0104_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0104_sticks.pdf}\\

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0326_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0326_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0326_sticks.pdf}&

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0330_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0330_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0330_sticks.pdf}\\

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1097_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1097_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1097_sticks.pdf}&

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1017_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1017_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1017_sticks.pdf}\\

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0950_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0950_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0950_sticks.pdf}&

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1652_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1652_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1652_sticks.pdf}\\

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0568_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0568_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0568_sticks.pdf}&

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0629_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0629_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0629_sticks.pdf}\\

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1589_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1589_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1589_sticks.pdf}&

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1183_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1183_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1183_sticks.pdf}\\

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0092_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0092_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0092_sticks.pdf}&

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1366_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1366_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1366_sticks.pdf}\\


  \end{tabular}
  \label{fig:qualitative_mpii_2}
\end{figure*}

\begin{figure*}
  \centering
  \begin{tabular}{c c c c c c}



\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0029_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0029_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0029_sticks.pdf}&

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0772_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0772_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0772_sticks.pdf}\\

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0832_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0832_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0832_sticks.pdf}&

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0635_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0635_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0635_sticks.pdf}\\

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0170_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0170_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0170_sticks.pdf}&

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0006_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0006_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0006_sticks.pdf}\\

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0094_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0094_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0094_sticks.pdf}&

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0903_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0903_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0903_sticks.pdf}\\

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1116_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1116_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1116_sticks.pdf}&

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0697_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0697_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0697_sticks.pdf}\\

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0210_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0210_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0210_sticks.pdf}&

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1033_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1033_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1033_sticks.pdf}\\

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0804_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0804_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0804_sticks.pdf}&

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0704_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0704_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0704_sticks.pdf}\\

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0075_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0075_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0075_sticks.pdf}&

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0472_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0472_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_0472_sticks.pdf}\\

\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1603_init_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1603_graph.pdf}&
\includegraphics[width=0.16\linewidth]{figures/mpii-supp/imgidx_1603_sticks.pdf}&

  \end{tabular}
  \label{fig:qualitative_mpii_3}
\end{figure*}


==> figure_qualitative_waf.tex <==
\begin{figure}
  \centering
  \begin{tabular}{c c c }
  \includegraphics[height=0.245\linewidth,width=0.45\linewidth]{figures/waf/imgidx_0005_sticks.pdf}&
  \includegraphics[height=0.245\linewidth,width=0.45\linewidth]{figures/waf/imgidx_0005_sticks_chen.pdf}\\
  \includegraphics[height=0.245\linewidth,width=0.45\linewidth]{figures/waf/imgidx_0007_sticks.pdf}&
  \includegraphics[height=0.245\linewidth,width=0.45\linewidth]{figures/waf/imgidx_0007_sticks_chen.pdf}\\
  \includegraphics[height=0.245\linewidth,width=0.45\linewidth]{figures/waf/imgidx_0014_sticks.pdf}&
  \includegraphics[height=0.245\linewidth,width=0.45\linewidth]{figures/waf/imgidx_0014_sticks_chen.pdf}\\

  \includegraphics[height=0.245\linewidth,width=0.45\linewidth]{figures/waf/imgidx_0053_sticks.pdf}&
  \includegraphics[height=0.245\linewidth,width=0.45\linewidth]{figures/waf/imgidx_0053_sticks_chen.pdf}\\

  \includegraphics[height=0.245\linewidth,width=0.45\linewidth]{figures/waf/imgidx_0063_sticks.pdf}&
  \includegraphics[height=0.245\linewidth,width=0.45\linewidth]{figures/waf/imgidx_0063_sticks_chen.pdf}\\
  \includegraphics[height=0.245\linewidth,width=0.45\linewidth]{figures/waf/imgidx_0097_sticks.pdf}&
  \includegraphics[height=0.245\linewidth,width=0.45\linewidth]{figures/waf/imgidx_0097_sticks_chen.pdf}\\
  \includegraphics[height=0.245\linewidth,width=0.45\linewidth]{figures/waf/imgidx_0119_sticks.pdf}&
  \includegraphics[height=0.245\linewidth,width=0.45\linewidth]{figures/waf/imgidx_0119_sticks_chen.pdf}\\
  \includegraphics[height=0.245\linewidth,width=0.45\linewidth]{figures/waf/imgidx_0135_sticks.pdf}&
  \includegraphics[height=0.245\linewidth,width=0.45\linewidth]{figures/waf/imgidx_0135_sticks_chen.pdf}\\
  \includegraphics[height=0.245\linewidth,width=0.45\linewidth]{figures/waf/imgidx_0174_sticks.pdf}&
  \includegraphics[height=0.245\linewidth,width=0.45\linewidth]{figures/waf/imgidx_0174_sticks_chen.pdf}\\
  
  \end{tabular}
  \vspace{-0.1em}
  \caption{ \textcolor{red}{Qualitative comparison on "We are the family" dataset.  Images from Chen and Yullie paper. {\it First
        column}: Results by our approach. {\it Second column}: corresponding results shown in \cite{Chen:2015:POC} .}
  } 
    \vspace{-1.2em}
  \label{fig:qualitative_waf}
\end{figure}


==> pck-torso-dense-expidx1.tex <==
VGG 420k +LSP-EXT softmax & 0  & 0  & 0  & 0  & 0  & 0 & 0 & 0 & 0 \\



==> pck-torso-expidx104.tex <==
scale 4, lr 0.004, step 320k, 1M, IoU pos 0.4, IoU reg 0.5, IoU min bg 0, add flipped& 89.3  & 79.1  & 67.8  & 61.0  & 72.8  & 72.5 & 65.2 & 69.3 & 72.5 & 44.3 \\



==> pck-torso-expidx118.tex <==
AlN lr0.004 \textbf{(500k) 2M} sc4 IoU0.4 augm& 88.4  & 79.7  & 69.2  & 62.1  & 73.3  & 72.0 & 65.6 & 70.3 & 72.9 \\



==> pck-torso-expidx144.tex <==
scale 4, lr 0.004, step 160k, 240k, IoU pos 0.4, IoU reg 0.5, IoU min bg 0, jitter 100-03-03, train lspet& 90.1  & 74.3  & 61.1  & 56.1  & 68.5  & 65.1 & 58.5 & 63.9 & 67.7 & 41.8 \\



==> pck-torso-expidx166.tex <==
\quad\quad + finetune LSP & 92.9  & 81.0  & 72.1  & 66.4  & 80.6  & 77.6 & 75.0 & 77.9 & 51.6\\



==> pck-torso-expidx179.tex <==
VGG lr0.004 (160k) \textbf{520M} sc4 IoU0.4 augm& 91.1  & 84.6  & 75.2  & 69.1  & 78.2  & 77.8 & 72.9 & 76.3 & 78.4\\



==> pck-torso-expidx227.tex <==
\quad\quad + \textit{no} bbox reg& 94.1  & 85.1  & 76.8  & 72.8  & 81.2  & 81.4 & 77.5 & 78.3 & 81.3 \\



==> pck-torso-expidx38.tex <==
scale 4, lr 0.003, step 160k, 240k, IoU pos 0.4, IoU reg 0.5& 87.5  & 75.5  & 63.8  & 56.5  & 68.8  & 66.9 & 59.4 & 65.3 & 68.3 \\



==> pck-torso-expidx383.tex <==
scale 4, lr 0.004, step 160k, 320k, finetune lsp, torso head, vgg& 94.6  & 85.5  & 77.4  & 71.4  & 83.9  & 80.8 & 77.5 & 78.1 & 81.6 & 55.5 & 97.3 & 92.4 \\



==> pck-torso-expidx505.tex <==
\quad+MPII-LSPET& 91.7  & 82.8  & 74.5  & 68.0  & 80.1  & 79.9 & 75.2 & 78.9 & 51.5\\



==> pck-torso-expidx507.tex <==
\quad\quad + finetune LSP lr0.0005 (10k) 40k & 94.7  & 85.2  & 76.8  & 71.0  & 82.5  & 82.2 & 78.2 & 81.5 & 55.4 \\



==> pck-torso-expidx508.tex <==
lr 0.004, mpii+lspet, finetune lsp, test lsp& 94.8  & 85.3  & 77.0  & 71.2  & 83.5  & 81.8 & 77.2 & 77.9 & 81.6 & 55.4 \\



==> pck-torso-expidx70.tex <==
scale 4, lr 0.003, step 160k, 240k, IoU pos 0.4, IoU reg 0.5, IoU min bg 0, jitter 100 pos 0.3 scale 0.3, finetune lsp 2000 lr-0001-lr-step-80k-140k-jitter-100-03-03& 91.7  & 78.6  & 68.6  & 63.7  & 78.1  & 74.2 & 69.4 & 70.3 & 74.9 & 49.1 \\



==> pck-torso-expidx9.tex <==
\quad scale 4 & 86.3  & 74.5  & 62.7  & 54.2  & 65.6  & 63.6 & 55.1 & 63.8 & 66.0 \\



==> pcp-expidx456.tex <==
Fast R-CNN~\multb~+ torso & 96.7 & 78.8 & 74.1 & 83.7 & 81.0 & 84.6 \\


==> pcp-expidx675.tex <==
%Dense \textit{MP100} & 96.7 & 78.9 & 80.6 & 77.3 & 78.9 & 83.7 & 82.7 & 84.7 \\
Dense \textit{MP100} & 96.7 & 79.8 & 78.1 & 83.7 & 82.7 & 84.7 \\


==> pcp-expidx685.tex <==
%Dense \textit{MP125} & 96.7 & 81.0 & 83.1 & 78.1 & 81.2 & 83.7 & 84.0 & 86.0 \\
Dense \textit{MP125} & 96.7 & \textbf{82.1} & \textbf{79.7} & 83.7 & \textbf{84.0} & \textbf{86.0} \\


==> pcp-torso-head-expidx456.tex <==
Fast R-CNN~\multb~+ torso eval& 90.9 & 78.8 &  74.1 & 83.8 & 80.1 & 84.7 \\


==> section_supplemental_mpii.tex <==
\section{Additional Results on MPII Single Person dataset}

\myparagraph{PCP evaluation measure.}


==> table_rcnn_unary_lsp.tex <==
%\renewcommand{\tabcolsep}{0.15cm}
\tabcolsep 1.0pt
\begin{table}[tbp]
 \scriptsize
  \centering
  \begin{tabular}{@{} l c ccc ccc cc@{}}
    \toprule
    Setting& Head   & Sho  & Elb & Wri & Hip & Knee & Ank & Up & Full\\
           &        &           &       &       &     &      &       & body  & body \\
    \midrule
    \input{experiments/pck-torso-expidx527-2.tex}
    \midrule
    \input{experiments/pck-torso-expidx534.tex}
    \midrule    
    \input{experiments/pck-torso-expidx0.tex}
    \input{experiments/pck-torso-expidx1.tex}
    \input{experiments/pck-torso-expidx26.tex}
    \input{experiments/pck-torso-expidx34.tex}
    \input{experiments/pck-torso-expidx98.tex}
    \input{experiments/pck-torso-expidx148.tex}
    \input{experiments/pck-torso-expidx118.tex}
    \input{experiments/pck-torso-expidx166.tex}
    \midrule
    \input{experiments/pck-torso-expidx176.tex} 
    %\input{experiments/pck-torso-expidx179.tex}
    \input{experiments/pck-torso-expidx201.tex}
    \input{experiments/pck-torso-expidx227.tex}
    \bottomrule
  \end{tabular}
  \caption[]{Unary only performance (PCK) of adapted Fast R-CNN on the LSP (Person-Centric) dataset.}
    \vspace{-0.5em}
  \label{tab:rcnn}
\end{table}

